Reinforcement Learning-Driven Adaptation Chains: A Robust Framework for Multi-Cloud Workflow Security

Cloud computing has emerged as a crucial solution for managing data- and compute-intensive workflows, offering scalability to address dynamic demands. However, security concerns persist, especially for workflows involving sensitive data and tasks. One of the main gaps in the literature is the lack of robust and flexible measures for reacting to these security violations. To address this, we propose an innovative approach leveraging Reinforcement Learning (RL) to formulate adaptation chains, responding effectively to security violations within cloud-based workflows. These chains consist of sequences of adaptation actions tailored to attack characteristics, workflow dependencies, and user-defined requirements. Unlike conventional single-task adaptations, adaptation chains provide a comprehensive mitigation strategy by taking into account both control and data dependencies between tasks, thereby accommodating conflicting objectives effectively. Moreover, our RL-based approach uses insights from past responses to mitigate uncertainties associated with adaptation costs. We evaluate the method using our jBPM and Cloudsim Plus based implementation and compare the impact of selected adaptation chains on workflows with the single adaptation approach. Results demonstrate that the adaptation chain approach outperforms in terms of total adaptation cost, offering resilience and adaptability against security threats.

==> Algorithms/AdaptationActionCostCalculation.tex <==

\begin{algorithm}
\caption{Adaptation Action Cost Calculation}
\label{alg:AdaptationActionCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w, ac $}
\Output{$P_{ac}, T_{ac}, V_{ac}, MS_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    $visitedParallelTasks \gets \emptyset$;\\
    \ForEach{$t_i$ in $ST$}{
        \If{$t_i \in \{t \mid aa_t \in ac\}$}{
            $ac_{price}+=P_{aa_{t_i}}$;\\
            $ac_{value}+=V_{aa_{t_i}}$;\\
            $ac_{mitigationScore}+=MS_{aa_{t_i},vt,a_k}$;\\
            \If{$parallelTasks_{t_i} \neq \emptyset$}{
                \If{$t_i \notin visitedParallelTasks$}{
                    $ac_{time}+=MAX(T_{aa_{t_i}},T_{parallelTasks})$;\\
                    $visitedParallelTasks \text{ }\cup= {t_i}$;\\
                 }
            }
            \Else{
                $ac_{time}+=T_{aa_{t_i}};$
            }
        }\Else{
            $ac_{price}+=Pdefault_{t_i}$;\\
            $ac_{value}+=Vdefault_{t_i}$;\\
            \If{$parallelTasks_{t_i} \neq \emptyset$}{
                 \If{$t_i \notin visitedParallelTasks$}{
                    $ac_{time}+=MAX(Tdefault_{t_i},T_{parallelTasks})$;\\
                    $visitedParallelTasks \text{ }\cup= {t_i}$;\\
                 }     
            }
            \Else{
                $ac_{time}+=Tdefault_{t_i};$
            }
        }
    }
}
\end{algorithm}



==> Algorithms/AdaptationChainCostCalculation.tex <==

\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation2}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC} $}
\Output{$\forall ac \in \mathcal{RAC}: time, price, value, mitigationScore$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    $visitedParallelTasks \gets \emptyset$;\\
    \ForEach{$t_i$ in $ST$}{
        \If{$t_i \in \{t \mid aa_t \in ac\}$}{
            $ac_{price}+=P_{aa_{t_i}}$;\\
            $ac_{value}+=V_{aa_{t_i}}$;\\
            $ac_{mitigationScore}+=MS_{aa_{t_i},vt,a_k}$;\\
            \If{$parallelTasks_{t_i} \neq \emptyset$}{
                \If{$t_i \notin visitedParallelTasks$}{
                    $ac_{time}+=MAX(T_{aa_{t_i}},T_{parallelTasks})$;\\
                    $visitedParallelTasks \text{ }\cup= {t_i}$;\\
                 }
            }
            \Else{
                $ac_{time}+=T_{aa_{t_i}};$
            }
        }\Else{
            $ac_{price}+=Pdefault_{t_i}$;\\
            $ac_{value}+=Vdefault_{t_i}$;\\
            \If{$parallelTasks_{t_i} \neq \emptyset$}{
                 \If{$t_i \notin visitedParallelTasks$}{
                    $ac_{time}+=MAX(Tdefault_{t_i},T_{parallelTasks})$;\\
                    $visitedParallelTasks \text{ }\cup= {t_i}$;\\
                 }     
            }
            \Else{
                $ac_{time}+=Tdefault_{t_i};$
            }
        }
    }
}
\end{algorithm}



==> Algorithms/AdaptationChainCostCalculation2.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},\mathcal{AC}_{history},W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: totalCost_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    \ForEach{$t_i$ in $ST$}{
        $aa_{current} \gets AA_{history} \gets aa_{vt} \gets\emptyset$;\\
        \If{$t_i \in \{t \mid aa_t \in ac\}$}{
            $aa_{current} \gets aa_{t_i}$;\\
        }
        \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
            \ForAll{$aa_{t_i}$}{
                $AA_{history} \gets AA_{history} \cup \{aa_{t_i}\}$;\\
            }
        }       
        \If{$aa_{current} \neq \emptyset$}{
            $ac_{P}+=P_{aa_{current}}$;\\
            $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
            $ac_{V}+=V_{aa_{current}}$;\\  
            $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
            $aa_{vt} \gets aa_{current}$;\\
        }
        \If{$AA_{history} \neq \emptyset$ }{
            \If{$t_i \in predecessors_{vt}$ }{
                \ForAll{$aa_{history}$ in $AA_{history}$}{
                    $ac_{P}+=P_{aa_{history}}$;\\
                    $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                    $ac_{V}+=V_{aa_{history}}$;\\
                    $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\
                }
            }
            \ElseIf{$aa_{current}== \emptyset $ }{
                $aa_{lowestCost} \gets LowestCostA(AA_{history}) $
                $ac_{P}+=P_{aa_{lowestCost}}$;\\
                $ac_{T}+=MAX(T_{aa_{lowestCost}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{lowestCost}}$;\\
                $ac_{MS}+=MS_{aa_{lowestCost},vt,a_k}$;\\
                $aa_{vt} \gets aa_{lowestCost}$;\\
            }

        }
        \If{$aa_{current}== \emptyset  \land AA_{history} == \emptyset$ }{
            $ac_{P}+=Pdefault_{t_i}$;\\
            $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
            $ac_{V}+=Vdefault_{t_i}$;\\
         }
         \If{$t_i== vt$}{
            Remove all adaptations except the $aa_{vt}$ from all chains($AA_{history}$ and $ac$)
         }
    }
      $totalCost_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$
}
\end{algorithm}


==> Algorithms/AdaptationChainCostCalculation2_1.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},\mathcal{ACL}_{history},W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: \phi_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $\phi_{ac}=\infty$;
    }
    \Else{
         \ForEach{$t_i$ in $(vt \cup pred_{vt})$}{
            $aa_{current} \gets AA_{history} \gets \emptyset$;\\
            \If{$t_i \in \{t \mid aa_t \in ac\}$}{
                $aa_{current} \gets aa_{t_i}$;\\
                \If{$t_i == vt$}{
                    Remove all other $aa_{vt}$ from $\mathcal{AC}_{history}$
                } 
            }
            \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
                \ForAll{$aa_{t_i}$}{
                    $AA_{history} \gets AA_{history} \cup \{aa_{t_i}\}$;\\
                }
            }  
            
            \If{$aa_{current} \neq \emptyset$}{
                $ac_{P}+=P_{aa_{current}}$;\\
                $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{current}}$;\\  
                $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
            }
            \If{$AA_{history} \neq \emptyset $  }{            
                    \ForAll{$aa_{history}$ in $AA_{history}$}{
                        $ac_{P}+=P_{aa_{history}}$;\\
                        $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                        $ac_{V}+=V_{aa_{history}}$;\\
                        $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\
                    }
            }
            \If{$aa_{current}== \emptyset  \land AA_{history} == \emptyset$ }{
                $ac_{P}+=Pdefault_{t_i}$;\\
                $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
                $ac_{V}+=Vdefault_{t_i}$;\\
             }
        
        }
    }
    $\phi_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
}
\end{algorithm}


==> Algorithms/AdaptationChainCostCalculation2_2.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},\mathcal{ACL}_{history},W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: \phi_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $\phi_{ac}=\infty$;
    }
    \Else{
         \ForEach{$t_i$ in $(vt \cup pred_{vt})$}{
            $aa_{current} \gets AA_{history} \gets \emptyset$;\\
            \If{$t_i \in \{t \mid aa_t \in ac\}$}{
                $aa_{current} \gets aa_{t_i}$;\\ 
                 \If{$t_i == vt$}{
                    Remove all other $aa_{vt}$ from $\mathcal{AC}_{history}$
                }
            }
            \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
                \ForAll{$aa_{t_i}$}{
                    $AA_{history} \gets AA_{history} \cup \{aa_{t_i}\}$;\\
                }
            }  
            
            \If{$aa_{current} \neq \emptyset$}{
                $ac_{P}+=P_{aa_{current}}$;\\
                $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{current}}$;\\  
                $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
            }

            \If{$t_i == vt \land aa_{current}== \emptyset  \land AA_{history} \neq \emptyset$ }{
                $aa_{history}$ \gets \text{last } $aa$ \text{ in } $AA_{history}$
                $ac_{P}+=P_{aa_{history}}$;\\
                $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{history}}$;\\
                $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\
                    
             }
          
            \If{$aa_{current}== \emptyset  \land AA_{history} == \emptyset$ }{
                $ac_{P}+=Pdefault_{t_i}$;\\
                $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
                $ac_{V}+=Vdefault_{t_i}$;\\
             }
        
        }
    }
    $\phi_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
}
\end{algorithm}


==> Algorithms/AdaptationChainCostCalculation3.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$\mathcal{RAC}_{vt,a_k},\mathcal{AC}_{history},Constraints,W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: totalCost_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
   \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $totalCost_{ac}=\infty$;
    }
    \Else{
    \ForEach{$t_i$ in $(vt \cup predecessors_{vt})$}{
        $aa_{current} \gets AA_{history} \gets \emptyset$;\\
        \If{$t_i \in \{t \mid aa_t \in ac\}$}{
            $aa_{current} \gets aa_{t_i}$;\\
        }
        \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
            \ForAll{$aa_{t_i}$}{
                $AA_{history} \gets AA_{history} \cup \{aa_{t_i}\}$;\\
            }
        }  
        
        \If{$aa_{current} \neq \emptyset$}{
            $ac_{P}+=P_{aa_{current}}$;\\
            $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
            $ac_{V}+=V_{aa_{current}}$;\\  
            $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
        }
        \If{$AA_{history} \neq \emptyset  $  }{            
                \ForAll{$aa_{history}$ in $AA_{history}$}{
                    $ac_{P}+=P_{aa_{history}}$;\\
                    $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                    $ac_{V}+=V_{aa_{history}}$;\\
                    $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\
                }
        }
        \If{$aa_{current}== \emptyset  \land AA_{history} == \emptyset$ }{
            $ac_{P}+=Pdefault_{t_i}$;\\
            $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
            $ac_{V}+=Vdefault_{t_i}$;\\
         }
        
    }
    $totalCost_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
    }

}

\end{algorithm}


==> Algorithms/AdaptationChainCostCalculation4.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$\mathcal{RAC}_{vt,a_k},\mathcal{ACL}_{history},Constraints,W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: \phi_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
   \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $\phi_{ac}=\infty$;
    }
    \Else{
        $aa_{current} \gets AA_{history} \gets \emptyset$;\\
        \If{$vt \in \{t \mid aa_t \in ac\}$}{
            $aa_{current} \gets aa_{vt}$;\\
        }
        \If{$ vt \in  \{t \mid \exists ac_h \in \mathcal{ACL}_{history}, aa_t \in ac_h\}$}{
            \ForAll{$aa_{vt}$}{
                $AA_{history} \gets AA_{history} \cup \{aa_{vt}\}$;\\
            }
        }  
        
        \If{$aa_{current} \neq \emptyset$}{
            $ac_{P}+=P_{aa_{current}}$;\\
            $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
            $ac_{V}+=V_{aa_{current}}$;\\  
            $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
        }
        \If{$AA_{history} \neq \emptyset  $  }{            
                \ForAll{$aa_{history}$ in $AA_{history}$}{
                    $ac_{P}+=P_{aa_{history}}$;\\
                    $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                    $ac_{V}+=V_{aa_{history}}$;\\
                    $ac_{MS}+=MS_{aa_{history},vt_{history},a_k}$;\\
                }
        }
        \If{$aa_{current}== \emptyset  \land AA_{history} == \emptyset$ }{
            $ac_{P}+=Pdefault_{vt}$;\\
            $ac_{T}+=MAX(T_{Tdefault_{vt}},T_{parallelTasks});$\\
            $ac_{V}+=Vdefault_{vt}$;\\
         }
        
    $\phi_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
    }

}

\end{algorithm}


Algorithm \ref{alg:AdaptationChainCostCalculation} details the process of computing the Adaptation Chain Cost for each adaptation chain ($ac$) in the set $\mathcal{RAC}$. In the initial step, the algorithm examines whether the introduction of the current chain ($ac$) would lead to a conflict with any of the Adaptation Chain Constraints as defined in Definition \ref{def:14}. If such a conflict is identified with any constraint $const$, the algorithm sets the total cost of the current $ac$ to infinity (lines 2-3). Otherwise, for the task $vt$ (the task for which we are currently determining the optimal adaptation chain),  the algorithm checks if the task contributes to the adaptation chain $ac$. This check involves determining if there exists an adaptation action ($aa_{current}$) that needs application in task $vt$ (lines 6-7). Subsequently, the algorithm examines whether there are any prior selected adaptations ($AA_{history}$) already applied to task $vt$ based on historical adaptations (lines 8-10). Given the potential for multiple adaptation actions to have been applied to task $vt$ based on prior selected adaptation chains, all viable options are included in the set $AA_{history}$.

If $aa_{current}$ is not empty, the price, time, value, and mitigation score of this adaptation are added to the current cost of $ac$ (lines 11-15). In case $AA_{history}$ is not empty, all costs of adaptations in $AA_{history}$ are added to the current cost of $ac$ as they have already been applied (lines 16-21). 

If both $aa_{current}$ and $AA_{history}$ are empty, indicating no planned adaptation for $vt$ in both the current chain and history, the default value for task $vt$ is added to the current cost of $ac$ to ensure the consideration of this task's cost in the overall cost (lines 22-25). Finally, the total cost of $ac$ is calculated using Equation \ref{eq:AdaptationChainCost} (line 26).

==> Algorithms/AdaptationChainCostCalculation5.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},\mathcal{ACL}_{history},W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: \phi_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $\phi_{ac}=\infty$;
    }
    \Else{
        \ForEach{$t_i$ in  ($succ_{previous_{vt}}\cap pred_{vt})$ }{
             $aa_{history} \gets \emptyset$;\\
             \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
                    $aa_{history} \gets aa_{t_i}$ from the last applied $ac$;\\
            } 
            \If{$aa_{history} \neq \emptyset $  }{            
                $ac_{P}+=P_{aa_{history}}$;\\
                $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{history}}$;\\
                $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\
                
            }
            \If{ $AA_{history} == \emptyset$ }{
                $ac_{P}+=Pdefault_{t_i}$;\\
                $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
                $ac_{V}+=Vdefault_{t_i}$;\\
             }
        }
        \ForEach{$t_i$ in $(vt \cup pred_{vt})$}{
        $aa_{current} \gets \emptyset$;\\
            \If{$t_i \in \{t \mid aa_t \in ac\}$}{
                $aa_{current} \gets aa_{t_i}$;\\
            }
            
            \If{$aa_{current} \neq \emptyset$}{
                $ac_{P}+=P_{aa_{current}}$;\\
                $ac_{T}+= MAX(T_{aa_{current}},T_{parallelTasks});$\\
                $ac_{V}+=V_{aa_{current}}$;\\  
                $ac_{MS}+=MS_{aa_{current},vt,a_k}$;\\
                 \If{$t_i == vt$}{
                    Remove all other $aa_{vt}$ from $\mathcal{AC}_{history}$
                } 
            }
            \If{$t_i == vt \land aa_{current} == \emptyset $  }{      
                \If{$aa_{history} \neq \emptyset$}{
                    $ac_{P}+=P_{aa_{history}}$;\\
                    $ac_{T}+=MAX(T_{aa_{history}},T_{parallelTasks});$\\
                    $ac_{V}+=V_{aa_{history}}$;\\
                    $ac_{MS}+=MS_{aa_{history},vt,a_k}$;\\ 
                    }
                \Else{
                    $ac_{P}+=Pdefault_{t_i}$;\\
                    $ac_{T}+=MAX(T_{Tdefault_{t_i}},T_{parallelTasks});$\\
                    $ac_{V}+=Vdefault_{t_i}$;\\
                }
            }
        }
    }
    $\phi_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
}
\end{algorithm}


==> Algorithms/AdaptationChainCostCalculation6.tex <==
\begin{algorithm}
\caption{Adaptation Chain Cost Calculation}
\label{alg:AdaptationChainCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},\mathcal{ACL}_{history},W_{P},W_{T},W_{V},W_{MS} $}
\Output{$\forall ac \in \mathcal{RAC}: \phi_{ac}$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    \If{$\exists const \in Constraints$ such that $const \text{ matches } (ac \cup AA_{history})$}{
        $\phi_{ac}=\infty$;
    }
    \Else{
        \ForEach{$t_i$ in  ($succ_{previous_{vt}}\cap pred_{vt})$ }{
             $aa_{history} \gets \emptyset$;\\
             \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history}, aa_t \in ac_h\}$}{
                    $aa_{history} \gets aa_{t_i}$ from the last applied $ac$;\\
            } 
            \If{$aa_{history} \neq \emptyset $  }{            
                $ac_{P,T,V,MS} \mathrel{+}= aa_{{history}_{P, T, V, MS}}$;\\
            }
            \If{ $AA_{history} == \emptyset$ }{
                $ac_{P,T,V,MS} \mathrel{+}= Default_{P, T, V, MS}$;\\
             }
        }
        \ForEach{$t_i$ in $(vt \cup pred_{vt})$}{
        $aa_{current} \gets \emptyset$;\\
            \If{$t_i \in \{t \mid aa_t \in ac\}$}{
                $aa_{current} \gets aa_{t_i}$;\\
            }
            
            \If{$aa_{current} \neq \emptyset$}{
            $ac_{P,T,V,MS} \mathrel{+}= aa_{{current}_{P, T, V, MS}}$;\\
                 \If{$t_i == vt$}{
                    Remove all other $aa_{vt}$ from $\mathcal{AC}_{history}$
                } 
            }
            \If{$t_i == vt \land aa_{current} == \emptyset $  }{      
                \If{$aa_{history} \neq \emptyset$}{

                $ac_{P,T,V,MS} \mathrel{+}= aa_{{history}_{P, T, V, MS}}$;\\
                    }
                \Else{
                    $ac_{P,T,V,MS} \mathrel{+}= Default_{P, T, V, MS}$;\\
                }
            }
        }
    }
    $\phi_{ac}=W_{P} \cdot ac_{P}+ W_{T} \cdot ac_{T} +W_{V} \cdot ac_{V} +W_{MS}\cdot ac_{MS}$;
}
\end{algorithm}


Algorithm \ref{alg:AdaptationChainCostCalculation} details the process of computing the Adaptation Chain Cost for each adaptation chain ($ac$) in the set $\mathcal{RAC}$. In the initial step, the algorithm examines whether the introduction of the current chain ($ac$) would lead to a conflict with any of the Adaptation Chain Constraints as defined in Definition \ref{def:14}.
\vspace{-24pt}
\input{Algorithms/AdaptationChainCostCalculation7}
\vspace{-24pt}
If such a conflict is identified with any constraint $const$, the algorithm sets the total cost of the current $ac$ to infinity (lines 2-3). Otherwise, for the task $vt$ (the task for which we are currently determining the optimal adaptation chain),  the algorithm checks if the task contributes to the adaptation chain $ac$. This check involves determining if there exists an adaptation action ($aa_{current}$) that needs application in task $vt$ (lines 6-7). Subsequently, the algorithm examines whether there are any prior selected adaptations ($AA_{history}$) already applied to task $vt$ based on historical adaptations (lines 8-10). Given the potential for multiple adaptation actions to have been applied to task $vt$ based on prior selected adaptation chains, all viable options are included in the set $AA_{history}$.

If $aa_{current}$ is not empty, the price, time, value, and mitigation score of this adaptation are added to the current cost of $ac$ (lines 11-15). In case $AA_{history}$ is not empty, all costs of adaptations in $AA_{history}$ are added to the current cost of $ac$ as they have already been applied (lines 16-21). 

If both $aa_{current}$ and $AA_{history}$ are empty, indicating no planned adaptation for $vt$ in both the current chain and history, the default value for task $vt$ is added to the current cost of $ac$ to ensure the consideration of this task's cost in the overall cost (lines 22-25). Finally, the total cost of $ac$ is calculated using Equation \ref{eq:AdaptationChainCost} (line 26).


==> Algorithms/AdaptationSecurityChainSetGeneration.tex <==
\begin{algorithm}
    \caption{Adaptation Chain Set Generation}

    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

    \Input{$\mathcal{AA}_{t_i}$ - Set of feasible adaptation actions for each task $t_i$ \\
            $MA_{\delta_{(a_k)}}$ - Set of adaptation actions tailored to the severity of the detected attack $a_k$ \\
            $DT_{vt}$ - Set of tasks in the workflow for virtual machine $vt$}
    \Output{$ \mathcal{A}\mathcal{C}_{vt,a_k}$:  The Adaptation Chain Set}

     $coveredTasks \gets \emptyset$;
 
    
    \BlankLine
    \For{ all $t_i$ in  $DT_{vt}$}{
        \If{$t_i \notin coveredTasks$}{
            $coveredTasks$.add($t_i$);\\
            \For{$aa$ in $(\mathcal{AA}_{t_i} \cap MA_{\delta_{(a_k)}})$}{
                $\mathcal{A}\mathcal{C}_{old} \gets \mathcal{A}\mathcal{C}$;\\
                $adapt_{new} \gets (action, task)$;\\
                $ac_{new}$.add($adapt_{new}$);\\
                $\mathcal{A}\mathcal{C}$.add($ac_{new}$);\\
    		\For{$ac$ in $\mathcal{A}\mathcal{C}_{old}$}{
    			 $check \gets false$;\\
    			\For{$adapt$ in $ac$} {
    				\If{$adapt$.getTask()=$adapt_{new}$.getTask()}{
    					$check \gets true$;\\
                        }
    		}
    		\If{ $check = false$} {
                    $ac$.add($adapt_{new}$);\\
    			$\mathcal{A}\mathcal{C}$.add($ac$);
    		}		
		}
        }
    }
}

\end{algorithm}





==> Algorithms/AdaptationSecurityChainSetGeneration1-1.tex <==
\begin{algorithm}
    \caption{Adaptation Chain Set Generation}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

   \Input{
    $\mathcal{AA}_{t_i}$: Adaptation actions for each task $t_i$ \\
    $MA_{\delta_{(a_k)}}$: Adaptation actions for attack $a_k$ with severity $\delta$ \\
    $DT_{vt}$: Security-Dependent Tasks for virtual machine $vt$
    }
    \Output{
        $\mathcal{AC}_{vt,a_k}$: The Adaptation Chain Set
    }

    $coveredTasks \gets \emptyset$;

    \BlankLine
    \For{all $t_i$ in $DT_{vt}$}{
        \If{$t_i \notin coveredTasks$}{
            $coveredTasks \gets coveredTasks \cup \{t_i\}$\;
            \For{$aa$ in $(\mathcal{AA}_{t_i} \cap MA_{\delta_{(a_k)}})$}{
                $\mathcal{AC}_{old} \gets \mathcal{AC}$\;
                $adapt_{new} \gets (aa, t_i)$\;
                $ac_{new} \gets \{adapt_{new}\}$\;
                $\mathcal{AC} \gets \mathcal{AC} \cup \{ac_{new}\}$\;
                \For{$ac$ in $\mathcal{AC}_{old}$}{
                    $check \gets \text{false}$\;
                    \For{$adapt$ in $ac$}{
                        \If{$\text{adapt.getTask()} = \text{adapt}_{new}.\text{getTask()}$}{
                            $check \gets \text{true}$\;
                        }
                    }
                    \If{$\neg check$}{
                        $ac \gets ac \cup \{adapt_{new}\}$\;
                        $\mathcal{AC} \gets \mathcal{AC} \cup \{ac\}$\;
                    }
                }
            }
        }
    }
\end{algorithm}



==> Algorithms/AdaptationSecurityChainSetGeneration2.tex <==
\begin{algorithm}
    \caption{Adaptation Chain Set Generation}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

   \Input{
    $\mathcal{AA}_{t_i}$, $MA_{\delta_{(a_k)}}$, $DT_{vt}$
    }
    \Output{
        $\mathcal{AC}_{vt,a_k}$
    }
    \BlankLine
    $\mathcal{AC} \gets \emptyset$;\\
    \For{$t_i$ in $DT_{vt}$}{
        \For{$aa_i$ in $(\mathcal{AA}_{t_i} \cap MA_{\delta_{(a_k)}})$}{
            $\mathcal{AC}_{new} \gets \mathcal{AC} \cup \{(t_i,aa_i)\}$\;
            \For{$ac$ in $\mathcal{AC}$}{
                $check \gets \text{true}$\;
                \For{$(t_j,aa_j)$ in $ac$}{
                    \If{$t_i==t_j$}{
                        $check \gets \text{false}$\;
                    }
                }
                \If{$check$}{
                    $ac \gets ac \text{\guillemotright}(t_j,aa_j)$\;
                    $\mathcal{AC}_{new} \gets \mathcal{AC}_{new} \cup \{ac\}$\;
                }
            }
            $\mathcal{AC} \gets \mathcal{AC}_{new}$;\\
        }
    }
\end{algorithm}



==> Algorithms/ApplySelectedAdaptationChain.tex <==
\begin{algorithm}
\scriptsize
\caption{Applying Selected Adaptation Chain}
\label{alg:ApplySelectedAdaptationChain}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,ac^*, current_{inst}$}
\Output{Applying $ac^*$ within $current_{inst}$}

\BlankLine
Suspend $current_{inst}$;\\
$t_{start}\gets vt$;\\
\ForEach{$t_i$ in $ pred_{vt}$}{
    \textbf{if }$t_i \in \{t \mid aa_t \in ac\}$ \textbf{ then } $t_{start}=t_i$ 
}
Resume $current_{inst} from t_{start}$;\\
\If{$t_{start} \neq vt$}{
    \ForEach{$t_j$ in $ {t_{start}  \cup Succ_{t_{start}}}$}{
        $aa_{current} \gets \emptyset$;\\
        \If{$t_j \in \{t \mid aa_t \in ac\}$}{
            $aa_{current} \gets aa_{t_j}$;\\
            Adapt $t_j$ with $aa_{current}$;\\
        }
        \Else{
            Repeat $t_j$;\\
        }
    }
}
\Else{
    \If{$vt \in \{t \mid aa_t \in ac\}$}{
            $aa_{current} \gets aa_{vt}$;\\
            Adapt $vt$ with $aa_{current}$;\\
        }
        \Else{
            Execute $vt$;\\
        }
    }
\end{algorithm}


==> Algorithms/ChainExample1.tex <==
\begin{equation*}
\begin{aligned}
&\{(t_1 \rightarrow \text{Insert})\}, \{(t_1 \rightarrow \text{Rework})\}, \{(t_1 \rightarrow \text{ReConfiguration})\}\\
&\{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_3 \rightarrow \text{Insert})\}, \{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_3 \rightarrow \text{Rework})\},\\
&\{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_3 \rightarrow \text{ReConfiguration})\},\\
&\{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_3 \rightarrow \text{Insert}) \text{\guillemotright}(t_4 \rightarrow \text{Insert}) \text{\guillemotright}(t_5 \rightarrow \text{Insert})\text{\guillemotright}(t_6 \rightarrow \text{Insert})\},\\
&\ldots
\end{aligned}
\end{equation*}


\textbf{Example 6:} Consider a scenario where a Denial of Service (DOS) attack with high severity occurs in task $t_5$. In this context, the Adaptation Security Chain Set is defined as:
\begin{equation*}
\begin{aligned}
\mathcal{A}\mathcal{C}_{t_5,a_{DOS}} = \prod_{\forall t_i \in DT_{t_5}} \biggl( \mathcal{AA}_{t_i} &\cap \{ \text{Insert, Rework,} \\
&\text{Redundancy, ReConfiguration} \} \biggr)
\end{aligned}
\end{equation*}

This product involves the intersection of adaptation actions $\mathcal{AA}_{t_i}$ and the set \{Insert, Rework, Redundancy, ReConfiguration\} for each task $t_i$ in the set $DT_{t_5}$. The resulting set is:
\begin{equation*}
\begin{aligned}
&\prod\biggl(\{(t_1\rightarrow\text{Insert}), (t_1 \rightarrow \text{Rework}), (t_1 \rightarrow \text{ReConfiguration})\},\\
&\{(t_3 \rightarrow \text{Insert}), (t_3 \rightarrow \text{Rework}), (t_3 \rightarrow \text{ReConfiguration})\},\\
&\{(t_4 \rightarrow \text{Insert}), (t_4 \rightarrow \text{Rework}), (t_4 \rightarrow \text{ReConfiguration})\},\\
&\{(t_5 \rightarrow \text{Insert}), (t_5 \rightarrow \text{Rework}), (t_5 \rightarrow \text{ReConfiguration})\},\\
&\{(t_6 \rightarrow \text{Insert}), (t_6 \rightarrow \text{Rework}), (t_6 \rightarrow \text{ReConfiguration})\}\biggr)
\end{aligned}
\end{equation*}


examples of cartesian combination of the above set that represents the potential adaptation actions in response to the DOS attack on $t_5$. are :
\input{manuscript/src/Algorithms/chainExample2}

==> Algorithms/RL.tex <==
\usepackage[ruled]{algorithm2e}

\begin{algorithm}
\caption{Adaptation Action Selection Algorithm}
\label{alg:AdaptationActionSelectionAlgorithm}
\SetAlgoNlRelativeSize{0}
\SetAlgoNlRelativeSize{-1}
\SetAlgoNlRelativeSize{1}
\SetAlgoNlRelativeSize{-2}
\SetAlgoNlRelativeSize{-1}
\SetAlgoNlRelativeSize{-2}

\KwIn{$l_{a_k}$, $BackupSrc_{t_i}$}
\KwOut{Selecting the suitable Adaptation Actions for the detected attack}

$attackScore \leftarrow ComputeAttackScore(a_k,t_i,s_j,l_{a_k})$ based on Equation \ref{eq:attack_score}\;

\If{$attackScore > Tenant.AdaptTriggerThresh$}{
    \eIf{Lowest-Cost Strategy}{
        $finalAA \leftarrow MA_{l_{(a_k)}} \cap AA_{t_i}$\;
        \ForEach{Adaptation Action $aa$ in $finalAA$}{
            $AC[aa] \leftarrow$ ComputeAdaptationCost($aa$, $t_i$) based on Equation \ref{eq:AdaptationCost}\;
        }
        Sort $AC$ in Ascending order\;
        $Selectedaa \leftarrow aa$ corresponds to the first item in $AC$\;
    }{
        \If{Adaptive Strategy}{
            $Selectedaa \leftarrow$ Predicted $aa$ based on $\mathcal{M}_{ActionSelection}$ (Algorithm \ref{alg:TrainingActionSelectionAlgorithm})\;
        }
    }
    \If{$Selectedaa \in$ tenant-level adaptation actions}{
        TenantAdaptation($Selectedaa$)\;
    }
    \Else{
        MiddlewareAdaptation($Selectedaa$)\;
    }
}
\end{algorithm}


==> Algorithms/SDM_Calculation.tex <==
\begin{algorithm}
\caption{Security Dependency Matrix ($SDM_w$) Calculation}
\label{alg:SecurityDependencyMatrix}
\begin{algorithmic}[1]
\REQUIRE $W$: Workflow represented as ($ST$, $D$, $E_c$, $E_d$)
\ENSURE $SDM_w$: Security Dependency Matrix for $W$

\STATE $SDM_w \gets$ initialize\_matrix($ST$) with zeros

\FOR{$t_i$ in $ST$}
    \FOR{$t_j$ in $ST$}
        \STATE  $C\gets0, I\gets0, A\gets0$
        \IF{ $t_i == t_j$}
            \STATE  $C\gets1, I\gets1, A\gets1$
        \ELSE
            \COMMENT{Confidentiality Impact}
            \IF{there is a backward or forward data flow connection between $t_i$ and $t_j$}
                \STATE $C \mathrel{+}= \prod_{\forall D_k \in \text{data flow connection}} Conf_{D_k}$
            \ENDIF

            \COMMENT{Integrity Impact}
            \IF{there is a forward data or control flow connection between $t_i$ and $t_j$}
                \STATE  $I$ \mathrel{+}= \prod_{\forall D_k \in \text{data flow connection}} Integrity_{D_k}$
            \ENDIF
             \IF{$t_j \in \text{DFCS}(t_i) \,||\, t_j \in \text{CFCS}(t_i) $}
                 \STATE $I = \prod_{\substack{t_k \\ t_i \leq t_k \leq t_j}} I_{t_k}$ 
            \ENDIF
    \IF{$t_j \in \text{DFCS}(t_i) \,||\, t_j \in \text{CFCS}(t_i) $}
                 \STATE $I = \prod_{\substack{t_k | t_i \leq t_k \leq t_j}} I_{t_k}$ 
            \ENDIF

             \IF{$t_j \in DFCS(t_i) \,||\, t_j \in CFCS(t_i) $}
                \STATE $I = \prod_{\forall t_k \, \text{such that} \, t_i \leq t_k \leq t_j} I_{t_k}$ 
            \ENDIF

             \COMMENT{Availability Impact}
             \IF{there is a forward data flow connection between $t_i$ and $t_j$}
                \STATE $A \mathrel{+}= \prod_{\forall D_k \in \text{data flow connection}} Availability_{D_k}$
            \ENDIF
         \ENDIF
        $SDM_w[t_i][t_j]\gets(C,I,A)
    \ENDFOR
\ENDFOR

\RETURN $SDM_w$
\end{algorithmic}
\end{algorithm}


==> Algorithms/SDM_Calculation1.tex <==
\begin{algorithm}
\caption{Security Dependency Matrix Computation}
\label{alg:SecurityDependencyMatrix}
\begin{algorithmic}[1]
\REQUIRE $W$: Workflow represented as ($ST$, $D$, $E_c$, $E_d$)
\ENSURE $SDM_w$: Security Dependency Matrix for $W$

\STATE $SDM_w \gets$ initialize\_matrix($ST$) with zeros

\FOR{$t_i$ in $ST$}
    \FOR{$t_j$ in $ST$}
        \STATE $C \gets 0, I \gets 0, A \gets 0$

        \IF{$t_i \neq t_j$}

            \IF{$t_j \in DFCS(t_i) \,||\, t_i \in DFCS(t_j) $}
                \STATE $C = \prod_{\substack{t_k \\ (t_i \leq t_k \leq t_j) \,||\, (t_j \leq t_k \leq t_i)}} C_{t_k}$ 

            \ENDIF

            \IF{$t_j \in \text{DFCS}(t_i) \,||\, t_j \in \text{CFCS}(t_i) $}
                \STATE $I = \prod_{\substack{t_k \\ t_i \leq t_k \leq t_j}} I_{t_k}$ 
            \ENDIF

            \IF{$t_j \in DFCS(t_i) $}
                \STATE $A = \prod_{\substack{t_k \\ t_i \leq t_k \leq t_j}} A_{t_k}$ 
            \ENDIF
        \ELSE
            \STATE $C \gets 1, I \gets 1, A \gets 1$
        \ENDIF

        \STATE $SDM_w[t_i][t_j] \gets (C, I, A)$
    \ENDFOR
\ENDFOR

\RETURN $SDM_w$
\end{algorithmic}
\end{algorithm}


==> Algorithms/SDM_Calculation2.tex <==
\begin{algorithm}
\caption{Security Dependency Matrix Computation}
\label{alg:SecurityDependencyMatrix}
\begin{algorithmic}[1]
\REQUIRE $W$: Workflow represented as ($ST$, $D$, $E_c$, $E_d$)
\ENSURE $SDM_w$: Security Dependency Matrix for $W$

\STATE $SDM_w \gets$ initialize\_matrix($ST$) with zeros

\FOR{$t_i$ in $ST$}
    \FOR{$t_j$ in $ST$}
        \IF{$t_i \neq t_j$}

            \IF{$t_j \in DFCS(t_i) \,||\, t_i \in DFCS(t_j) $}
                \STATE $C_{ij} = \prod_{\substack{t_k \\ (t_i \leq t_k \leq t_j) \,||\, (t_j \leq t_k \leq t_i)}} C_{t_k}$ 

            \ENDIF

            \IF{$t_j \in \text{DFCS}(t_i) \,||\, t_j \in \text{CFCS}(t_i) $}
                \STATE $I_{ij} = \prod_{\substack{t_k \\ t_i \leq t_k \leq t_j}} I_{t_k}$ 
            \ENDIF

            \IF{$t_j \in DFCS(t_i) $}
                \STATE $A_{ij} = \prod_{\substack{t_k \\ t_i \leq t_k \leq t_j}} A_{t_k}$ 
            \ENDIF
        \ELSE
            \STATE $C_{ij} \gets 1, I_{ij} \gets 1, A_{ij} \gets 1$
        \ENDIF

        \STATE $SDM_w[t_i][t_j] \gets (C_{ij}, I_{ij}, A_{ij})$
    \ENDFOR
\ENDFOR

\RETURN $SDM_w$
\end{algorithmic}
\end{algorithm}


==> Algorithms/WorkflowAdaptationCostCalculation.tex <==

\begin{algorithm}
\caption{Workflow Adaptation Cost Calculation}
\label{alg:WorkflowAdaptationCostCalculation}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{$w,\mathcal{RAC}_{vt,a_k},AC_{history} $}
\Output{Adaptation cost for $w$}

\BlankLine
\ForEach{$ac$ in $\mathcal{RAC}$}{
    $visitedParallelTasks \gets \emptyset$;\\
    \ForEach{$t_i$ in $ST$}{
        \If{$t_i \in \{t \mid aa_t \in ac\}$}{
            $condition_1=true$;\\
            $\text{currentAdapt}=aa_t$
        }
        \If{$ t_i \in  \{t \mid \exists ac_h \in \mathcal{AC}_{history} , aa_t \in ac_h\}$}{
            $condition_2=true$;\\
            $\text{plannedAdapt}=aa_t$
        }
        \If{$!condition_1 \text{ }\&\& \text{ }\ !condition_2$}{
            $ac_{price}+=Pdefault_{t_i}$;\\
            $ac_{value}+=Vdefault_{t_i}$;\\
            $ac_{time}+=ComputeTime(Tdefault_{t_i});$
        }
        \If{$condition_1 \text{ }\&\& \text{ }\ !condition_2$}{
        $ac_{price}+=P_{\text{currentAdapt}_{t_i}}$;\\
        $ac_{value}+=V_{\text{currentAdapt}_{t_i}}$;\\
        $ac_{time}+=ComputeTime(\text{currentAdapt}_{t_i});$
        $ac_{mitigationScore}+=MS_{\text{currentAdapt}_{t_i},vt,a_k}$;\\
        }
        \If{$!condition_1 \text{ }\&\& \text{ }\ condition_2$}{
             $ac_{price}+=P_{\text{plannedAdapt}_{t_i}}$;\\
             $ac_{value}+=V_{\text{plannedAdapt}_{t_i}}$;\\
             $ac_{time}+=ComputeTime(\text{plannedAdapt}_{t_i});$
             $ac_{mitigationScore}+=MS_{\text{plannedAdapt}_{t_i},vt,a_k}$;\\
        }
        \If{$condition_1 \text{ }\&\& \text{ }\ condition_2$}{
            \If{$t_i \in precedingTasks_vt$}{
             $ac_{price}+=P_{\text{plannedAdapt}_{t_i}}+P_{\text{currentAdapt}_{t_i}}$;\\
             $ac_{value}+=V_{\text{plannedAdapt}_{t_i}}+V_{\text{currentAdapt}_{t_i}}$;\\
             $ac_{time}+=ComputeTime(\text{plannedAdapt}_{t_i})+ComputeTime(\text{currentAdapt}_{t_i});$
             $ac_{mitigationScore}+=MS_{\text{plannedAdapt}_{t_i},vt,a_k}+MS_{\text{currentAdapt}_{t_i},vt,a_k}$;\\
            }
            \Else{
                $ac_{price}+=P_{\text{currentAdapt}_{t_i}}$;\\
                $ac_{value}+=V_{\text{currentAdapt}_{t_i}}$;\\
                $ac_{time}+=ComputeTime(\text{currentAdapt}_{t_i});$
                $ac_{mitigationScore}+=MS_{\text{currentAdapt}_{t_i},vt,a_k}$;\\
            }
        }
         
    }
}
\end{algorithm}



==> Algorithms/chainExample2.tex <==
\begin{equation*}
\begin{aligned}
&ac_1: \{(t_5 \rightarrow \text{Insert})\}\\
&ac_2: \{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_5 \rightarrow \text{Rework})\}\\
&ac_3:\{(t_3 \rightarrow \text{Insert})  \text{\guillemotright} (t_5 \rightarrow \text{ReConfiguration})\text{\guillemotright}(t_6 \rightarrow \text{Rework})\}\\
&ac_4: \{(t_1 \rightarrow \text{Insert})  \text{\guillemotright} (t_3 \rightarrow \text{Rework}) \text{\guillemotright}(t_4 \rightarrow \text{Insert}) \\
&\hspace{2em}\text{\guillemotright}(t_5 \rightarrow \text{Insert}) \text{\guillemotright}(t_6 \rightarrow \text{Rework})\}
\end{aligned}
\end{equation*}

==> figures/ADM.tex <==

\begin{figure*}
    \begin{align*}
        \begin{bNiceMatrix}[first-col,first-row]
            &t_1&t_2&t_3&t_4&t_5&t_6&t_7&t_8\\
            t_1& \text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.3,0.2,0.5} & \text{\scriptsize 0.1,0.1,0.3} & \text{\scriptsize 0,0,0.1} & \text{\scriptsize 0,0,0}\\
            t_2&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0.5,0.5} &\text{\scriptsize 0.3,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_3&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.3,0.5,0.5} &\text{\scriptsize 0.2,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_4&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.3,0.5,0.5} &\text{\scriptsize 0.2,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_5&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,1,0.5} &\text{\scriptsize 0.3,1,0.3} &\text{\scriptsize 0,0,0}\\
            t_6&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0.5,0.1} &\text{\scriptsize 0,0,0}\\
            t_7&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0,0,0}\\
            t_8&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.1,0,0} &\text{\scriptsize 0.1,0,0} &\text{\scriptsize 0,0,0} &\text{\scriptsize 1,1,1}\\
        \end{bNiceMatrix}
    \end{align*}
    \caption{Your matrix caption goes here.}
\end{figure*}



==> figures/SDM.tex <==
    \begin{align*}
        \begin{bNiceMatrix}[first-col,first-row]
            &t_1&t_2&t_3&t_4&t_5&t_6&t_7&t_8\\
            t_1& \text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.5,0.3,0.7} & \text{\scriptsize 0.3,0.2,0.5} & \text{\scriptsize 0.1,0.1,0.3} & \text{\scriptsize 0,0,0.1} & \text{\scriptsize 0,0,0}\\
            t_2&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0.5,0.5} &\text{\scriptsize 0.3,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_3&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.3,0.5,0.5} &\text{\scriptsize 0.2,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_4&\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.3,0.5,0.5} &\text{\scriptsize 0.2,0.3,0.3} &\text{\scriptsize 0.1,0.1,0.1} &\text{\scriptsize 0,0,0}\\
            t_5&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,1,0.5} &\text{\scriptsize 0.3,1,0.3} &\text{\scriptsize 0,0,0}\\
            t_6&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.5,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0.5,0.5,0.1} &\text{\scriptsize 0,0,0}\\
            t_7&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 1,1,1} &\text{\scriptsize 0,0,0}\\
            t_8&\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.3,0,0} &\text{\scriptsize 0.1,0,0} &\text{\scriptsize 0.1,0,0} &\text{\scriptsize 0,0,0} &\text{\scriptsize 1,1,1}\\
        \end{bNiceMatrix}
    \end{align*}



==> figures/SDM2.tex <==
\begin{align*}
    \begin{bNiceMatrix}[first-col,first-row]
        & t_1 & t_3 & t_4 & t_5 & t_6 & t_8 \\
        t_1 & \text{\scriptsize 1.0, 1.0, 1.0} & \text{\scriptsize 0.0, 1.0, 0.0} & \text{\scriptsize 0.0, 1.0, 0.0} & \text{\scriptsize 0.0, 1.0, 0.0} & \text{\scriptsize 0.0, 1.0, 0.0} & \text{\scriptsize 0.0, 0.1, 0.0} \\
        t_3 & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 1.0, 1.0, 1.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.25, 1.0, 1.0} & \text{\scriptsize 0.25, 1.0, 1.0} & \text{\scriptsize 0.0, 0.1, 0.0} \\
        t_4 & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 1.0, 1.0, 1.0} & \text{\scriptsize 0.35, 1.0, 0.5} & \text{\scriptsize 0.35, 1.0, 0.5} & \text{\scriptsize 0.0, 0.1, 0.0} \\
        t_5 & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.25, 0.0, 0.0} & \text{\scriptsize 0.25, 0.0, 0.0} & \text{\scriptsize 1.0, 1.0, 1.0} & \text{\scriptsize 0.5, 1.0, 1.0} & \text{\scriptsize 0.0, 0.1, 0.0} \\
        t_6 & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.5, 0.0, 0.0} & \text{\scriptsize 0.5, 0.0, 0.0} & \text{\scriptsize 1.0, 0.0, 0.0} & \text{\scriptsize 1.0, 1.0, 1.0} & \text{\scriptsize 0.0, 0.1, 0.0} \\
        t_8 & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 0.0, 0.0, 0.0} & \text{\scriptsize 1.0, 1.0, 1.0} \\
    \end{bNiceMatrix}
\end{align*}


==> tables/AttackSpecifications2.tex <==
\vspace*{-.4cm}
\begin{tabulary}{\linewidth}{p{1cm}p{2cm}p{2.2cm}p{3cm}p{6cm}}
 \textbf{} & \textbf{Impact on} &   \multicolumn{2}{c}{\textbf{Mitigation Actions}} & \textbf{}\\ 
% \multicolumn{3}{c}{\textbf{Mitigation Actions}}
  \textbf{AT} &
 \textbf{ (C,I,A)} &

\textbf{(Low,} &
\textbf{Medium,}&
\textbf{High)} 
\\  \hline  \hline
\textbf{DoS} &
(0.56,0.56,0.56)	&Switch, Rework	&Insert, Rework 	&Insert, Rework, Redundancy, ReConfiguration
\\  \hline

\textbf{Probe} &
(0.22,0.22,0)&	Skip&	 Skip, ReConfiguration& 	Skip, ReConfiguration
\\  \hline

 \textbf{U2R} &
(0.56,0.22,0.22)	&Insert, Rework 	&  Insert, Rework	& Insert, Rework, Redundancy, ReConfiguration
\\  \hline

 \textbf{R2L} &
0.56,0.56,0.22)&	Rework&	Insert, Rework &	 Insert, Rework, ReConfiguration
\\  \hline

\bottomrule 
\end{tabulary}\par 
\vspace*{-.4cm}



==> tables/Table1.tex <==
\begin{table*}[ht]
\caption{Possible Attacks in the Workflows}
\centering
\begin{tabular}{p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}}
\hline
Type of Attack & Related Attacks & Potential Targets in Workflow  & Implications of attacks \\
\hline
Application-based Attack & Fault injection, Inference Attack,
Account Hijacking, web service and protocol based attacks

& Fragment(group of tasks)
Data(Input/Output)
Message(Send/Receive)
Task(Code/Service), Control Flow Connector & Malicious manipulation of data,
Violation of data protection,
Denial-of-service\\

\hline

Network-based Attack &   port scanning, botnets, spoofing attacks, eavesdropping attack,the man-in-the-middle attack, and the replay attack     & Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) &
Violation of data protection,
Denial-of-service
 \\
\hline


VM-based Attack & Cross VM   side channel attacks
VM creation attacks
VM migration and roll back attacks
VM scheduler based attacks(VM escape, VM hopping, etc.) &
Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) & Violation of data protection
Denial-of-service  \\
\hline
\end{tabular}
\end{table*}


==> tables/adaptationActions.tex <==
%\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\vspace*{-.4cm}
\begin{tabulary}{\linewidth}{ 
p{1.7cm} p{2cm} p{1cm} p{1cm} p{1cm}}

\textbf{AdaptType} &
\textbf{T}  &
\textbf{P}  & 
\textbf{V}  &
\textbf{MI(C,I,A)}
\\  \hline  \hline

\textbf{Insert} &
$T_{newTask}$ & $P_{newTask}$ & $V_{newTask}$ &  $(0.7,0.9,0.9)$
\\  \hline

\textbf{Switch} &
$T_{Switch}$ & $P$  &  $V_{Switch}$ & $(0.7,0.6,0.8)$
\\  \hline

\textbf{Skip} &
$0$  & $0$ &  $0$ & $(0.5,0.4,0.6)$ 
\\  \hline

\textbf{Rework} &
$T_{BackupSrc}$  & $P_{BackupSrc}$ & $V$ & $(0.5,0.9,0.7)$
\\  \hline

\textbf{Redundancy} &
 $Max(T_{BackupSrc},T)$ & $P+P_{BackupSrc}$ & $V+V_{Redundancy}$ & $(0.5,0.8,0.9)$
\\  \hline

\textbf{Reconfiguration} &
$T+T_{reconfig}$ & $P+P_{reconfig}$ & $V+V_{Reconfig}$ & $(0.6,0.7,0.5)$
\\  \hline


\bottomrule 
\end{tabulary}\par 
\vspace*{-.4cm}


==> tables/adaptationActions2.tex <==
%\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\vspace*{-.4cm}
\begin{tabulary}{\linewidth}{ 
p{2.5cm} p{3.8cm} p{3cm} p{3.3cm} p{2cm}}

 \textbf{AdaptType} &
 \textbf{T}  &
\textbf{P}  & 
\textbf{V}  &
\textbf{MI(C,I,A)}
\\  \hline  \hline

\textbf{Insert} &
$T_{newTask}$ & $P_{newTask}$ & $V_{newTask}$ &  $(0.7,0.9,0.9)$
\\  \hline

\textbf{Switch} &
$T_{Switch}$ & $P$  &  $V_{Switch}$ & $(0.7,0.6,0.8)$
\\  \hline

\textbf{Skip} &
$0$  & $0$ &  $0$ & $(0.5,0.4,0.6)$ 
\\  \hline

\textbf{Rework} &
$T_{BackupSrc}$  & $P_{BackupSrc}$ & $V$ & $(0.5,0.9,0.7)$
\\  \hline

\textbf{Redundancy} &
 $Max(T_{BackupSrc},T)$ & $P+P_{BackupSrc}$ & $V+V_{Redundancy}$ & $(0.5,0.8,0.9)$
\\  \hline

\textbf{Reconfiguration} &
$T+T_{reconfig}$ & $P+P_{reconfig}$ & $V+V_{Reconfig}$ & $(0.6,0.7,0.5)$
\\  \hline


\bottomrule 
\end{tabulary}\par 
\vspace*{-.4cm}


==> tables/relatedWorks.tex <==
\vspace*{-.3cm}
%\begin{tabulary}{\linewidth}{  p{1.4cm} p{1.5cm}  p{2cm}  p{2.0cm} p{2.4cm}  p{2.4cm}  }
\begin{tabulary}{\linewidth}{>{\centering\arraybackslash}p{2cm}>{\centering\arraybackslash}p{1.7cm}>{\centering\arraybackslash}p{2.0cm}>{\centering\arraybackslash}p{3cm}>{\centering\arraybackslash}p{3cm}}
\hline
\textbf{Paper} & \textbf{Workflow Type} &  \textbf{Considered Security Objectives} & \textbf{Considered \newline Attacks} &  \textbf{Adaptation \newline Options} \\
\hline \hline
\cite{HosseiniShirvani2020}, 2020 & Business  & CIA & VM-based, \newline Network attacks & Static Trust \newline Calculation \\
\hline
\cite{Wang2020b}, 2020 \newline \cite{Wang2021}, 2021 & Scientific &  I & VM-based \newline attacks & Redundancy \\
\hline
\cite{Wen2020b}, 2020 & Scientific  & A & Clouds fail & Rescheduling the uncompleted tasks \\
\hline
\cite{Abazari2019}, 2018 & Scientific  & CIA & VM-based \newline attacks & Rescheduling the affected tasks \\
\hline
\cite{Ahmad2021}, 2021 & Scientific  & A & Hardware and \newline Software faults & Re-work \\
\hline
\cite{Alaei2021b}, 2021 & Scientific & A & Unavailability \newline of VMs & Re-work \\
\hline
\cite{soveizi2023enhancing}, 2023 & Scientific/Business & CIA & DoS,Probe,U2R,R2L  & Single Adaptation \\
\hline \bottomrule 
\end{tabulary}
\vspace*{-.4cm}

==> tables/table1-v2.tex <==
%\begin{tabular}{p{3cm} p{5cm} p{7cm}}
%\begin{tabular}{|p{0.15\linewidth}|p{0.15\linewidth}|p{0.6\linewidth}|}
\begin{tabulary}{\linewidth}{ p{0.05\linewidth}|p{0.15\linewidth}|p{0.2\linewidth}| p{0.5\linewidth}}
 \hline
\textbf{Attack Type} & \textbf{Attack Target} & \textbf{Malicious Party} &\textbf{Attack Scenario} \\
\hline
DOS  & Task: Receive Claim & Malicious Tenant/External Attacker & A coordinated Denial of Service (DOS) attack orchestrated by a rival company with the intention of disrupting the claims processing system \\
\hline
R2L  & Task/Intermediate data: Acquire  Hospital Report/Acquire Police Report & Malicious Workflow User/ Malicious Tenant&  Unauthorized access for the purpose of manipulating incident details with malicious intent \\
\hline
U2R  & Task/Intermediate data: Expert Claim Assessment & Malicious Workflow User& Exploits vulnerabilities to gain unauthorized access with the intention of altering reimbursement decisions \\
\hline
Probe  & Tenant’s Metadata/Users’ Metadata/Logic& Malicious Provider (Semi-Trusted)/Malicious Tenant& Gain access to observe process logic, decision criteria, and involved parties, accumulating intelligence about the reimbursement process, potentially for misuse or, more broadly, to access sensitive data within the process, such as customer information\\
\hline
\end{tabulary}\par 
% \end{tabular}


==> tables/variables.tex <==
predecessor tasks of the task $t_i$ ($pred_{t_i}$) refer to all tasks that must be completed before the task $t_i$  can start.
the predecessor tasks of task $t$ refer to the tasks that must be completed before task $t$ can start.

 the successors of task $t$ refers to the tasks that rely on the completion of task $t$ to start.
